SwiftNet: Using Graph Propagation as Meta-knowledge to Search Highly Representative Neural Architectures

Designing neural architectures for edge devices is subject to constraints of accuracy, inference latency, and computational cost. Traditionally, researchers manually craft deep neural networks to meet the needs of mobile devices. Neural Architecture Search (NAS) was proposed to automate the neural architecture design without requiring extensive domain expertise and significant manual efforts. Recent works utilized NAS to design mobile models by taking into account hardware constraints and achieved state-of-the-art accuracy with fewer parameters and less computational cost measured in Multiply-accumulates (MACs). To find highly compact neural architectures, existing works relies on predefined cells and directly applying width multiplier, which may potentially limit the model flexibility, reduce the useful feature map information, and cause accuracy drop. To conquer this issue, we propose GRAM(GRAph propagation as Meta-knowledge) that adopts fine-grained (node-wise) search method and accumulates the knowledge learned in updates into a meta-graph. As a result, GRAM can enable more flexible search space and achieve higher search efficiency. Without the constraints of predefined cell or blocks, we propose a new structure-level pruning method to remove redundant operations in neural architectures. SwiftNet, which is a set of models discovered by GRAM, outperforms MobileNet-V2 by 2.15x higher accuracy density and 2.42x faster with similar accuracy. Compared with FBNet, SwiftNet reduces the search cost by 26x and achieves 2.35x higher accuracy density and 1.47x speedup while preserving similar accuracy. SwiftNetcan obtain 63.28% top-1 accuracy on ImageNet-1K with only 53M MACs and 2.07M parameters. The corresponding inference latency is only 19.09 ms on Google Pixel 1.

==> backup_2_related_work_.tex <==
\section{RELATED WORK}

Some common approaches to improve the performance of NAS include: 
\subsection{Improving search algorithm}
A search algorithm decides in what way the searching space is going to be explored. It can be divided into two mainstreams:
\paragraph{Reinforcement Learning(RL)}
Some early works\cite{zoph2016neural} used RL to learn how to produce a good network. However, RL usually brings too much computation complexity and reduces the search time. Some recent work tries to improve this problem by weight sharing\cite{liu2018darts,zoph2018learning,pham2018efficient}. However, the result sacrifice architectural flexibility and did not consider hardware friendly. The most recent work\cite{wu2018fbnet,liu2019auto} takes these problems into consideration and get some more promising results. We will have further discuss of these two works in the following sections.
\paragraph{Evolutionary Algorithm(EA)}
EA by its definition is suitable for generating good performance networks. Some works\cite{real2017large,real2018regularized,liu2017hierarchical} using EA and produce good results. However, EA also has high computation cost, and usually been criticized as not robust enough. The quality of its final result is not stable due to random mutation. The work\cite{real2018regularized}also used cell lever exploration to shrink search space. And to tackle with the robustness problem, the works\cite{dong2018dpp,liu2018progressive} use sequential-model based optimization。
\paragraph{Gradient-based methods}
To shrink the search space and find a optimal solution faster, some works\cite{wu2018fbnet,liu2018progressive,luo2018neural,liu2018darts} are inspired by differentiable methods.
\subsection{Search acceleration}
\paragraph{Hypernetwork} Instead of train every child network from scratch, people use hypernetwork\cite{ha2016hypernetworks,brock2017smash,zhang2018graph} to approximate the optimal parameters of a sampled network, and estimate the child network's performance directly. By generating weights instead of training from scratch, hypernetworks are good initializers for child networks.
\subsection{Multi-objective NAS}
Not only accuracy, people also care about a networks' performance in other factors like inference latency, energy efficiency and memory usage. Some work are focusing on including these factors into training process.


==> unused.tex <==
%
A closed-form expression of the lower-bound of our search space size
$${(\sum_{i=1}^{n} C_{n-1}^{i})}^{(m\cdot h)}$$
Here n, m, h has the same meaning as described in Proposed Approach section

\begin{table*}[]
\centering
\begin{tabular}{cccccc}
\hline
Model & Method & Direct        & Scaling    & Latency(ms) & Top-1         \\ 
      &        & metrics based & complexity &             & accuracy (\%)\\ \hline
MobileNetV2 1.3x &Manual &-- &-- &33.8 &74.4 \\
ShuffleNetV2 2.0x  &Manual &Y &-- &33.3 &74.9 \\
ChamNet-A &EES &Y &$O(m + n)$ &29.8 &75.4 \\
\hline
MobileNetV2 1.0x &Manual &-- &-- &21.7 &71.8\\
ShuffleNetV2 1.5x  &Manual &Y &-- &22.0 &72.6\\
CondenseNet (G=C=4)  &Manual &-- &-- &28.7∗ &73.8\\
MnasNet 1.0x &RL &Y &$O(m · n · k)$ &23.8 &74.0\\
AMC  &RL &Y &$O(m · n · k)$ &-- &--\\
MorphNet  &Regularization &N &$O(m · n · k)$ &-- &--\\
ChamNet-B &EES &Y &$O(m + n)$ &19.9 &73.8\\
\hline
MobileNetV2 0.75x  &Manual &-- &-- &16.6 &69.8\\
ShuffleNetV2 1.0x  &Manual &Y &-- &14.9 &69.4\\
MnasNet 0.75x &RL &Y &$O(m · n · k)$ &18.4 &71.5\\
NetAdapt  &Pruning &Y &$O(m · k + n)$ &16.6 (63.6+) &70.9\\
ChamNet-C &EES &Y &$O(m + n)$ &15.0 &71.9\\
\hline
MobileNetV2 0.5x &Manual &-- &-- &10.6 &65.4\\
MnasNet 0.35x &RL &Y &$O(m · n · k)$ &10.7 &62.4\\
ChamNet-D &EES &Y &$O(m + n)$ &10.0 &69.0\\
\hline
MobileNetV2 0.35x &Manual &-- &-- &9.3 &60.3\\
ShuffleNetV2 0.5x &Manual &Y &-- &8.8 &60.3\\
ChamNet-E &EES &Y &$O(m + n)$ &6.1 &64.1\\
\hline
\end{tabular}
\end{table*}



\begin{table*}[]
\centering
\begin{tabular}{cccccc}
\hline
Module & Input Size & Output Size & filter size/stride & depth  \\ \hline
Image & $96 \times 96 \times 3$ &$96 \times 96 \times 3$ &-- & --  \\
\\ \hline
Conv-1 & $96 \times 96 \times 3$ &$48 \times 48 \times 64$ &$7 \times 7$\ /\ 2 & 64  \\
\\ \hline
Conv-2 & $48 \times 48 \times 64$ &$24 \times 24 \times 64$ &$3 \times 3$\ /\ 2 & 64  \\
\\ \hline
Meta-graph proposed architecture & $24 \times 24 \times 64$ &$3 \times 3 \times k$ & -- & --  \\
\\ \hline
Conv-identity & $3 \times 3 \times k$ &$3 \times 3 \times 1000$ &$1 \times 1$ & 1000  \\
\\ \hline
Average Pooling & $3 \times 3 \times 1000$ &$1 \times 1 \times 1000$ &-- & --  \\
\\ \hline
Flatten \& Prediction & $1 \times 1 \times 1000$ & $1000$ &-- & --  \\
\\ \hline

\end{tabular}
\caption{Architecture used for ImageNet Classification}
\end{table*}

\subsection{Pruning \& Quantization}
\cite{wen2016learning}
Our work can be paralleled with pruning and quantization to best realize compression on our model. Our method removes the unnecessary or weak operations in the computational graph, while pruning eliminates weights which is of no use or has little contribution to the results. This is also a kind of similarity between structure-level pruning and weight pruning. In addition, Quantization removes the redundancy in the computational precision, and it can also be combined with our work to compress the model size. The effects of pruning and quantization will be deeply studied in our future work.
